Gradient Localization Improves Lifelong Pretraining of Language Models

Large Language Models (LLMs) trained on web-scale text corpora have been shown to capture world knowledge in their parameters. However, the mechanism by which language models store different types of knowledge is poorly understood. In this work, we examine two types of knowledge relating to temporally sensitive entities and demonstrate that each type is localized to different sets of parameters within the LLMs. We hypothesize that the lack of consideration of the locality of knowledge in existing continual learning methods contributes to both: the failed uptake of new information, and catastrophic forgetting of previously learned information. We observe that sequences containing references to updated and newly mentioned entities exhibit larger gradient norms in a subset of layers. We demonstrate that targeting parameter updates to these relevant layers can improve the performance of continually pretraining on language containing temporal drift.

==> sections/5_analysis.tex <==
\section{Analysis}
Typically, it is common to train the full model or only the initial or final layer when adapting a pretrained model during finetuning or continual pretraining of a model from a pretrained initialization. In contrast to previous work, 

% 1.  Continual pretraining solely on knowledge changes is insufficient; All models exhibit distortion without sufficient regularization

    Rather than focusing on the exact neurons that correspond to a 

We observe that continual pretraining with our proposed method improves 


\subsection{Seen vs unseen entities.}

\subsection{Catastrophic Forgetting}



